Multi-Lingual Development & Programming Languages Interoperability: An Empirical Study

As part of a research on a novel in-process multiprogramming-language interoperability system, this study investigates the interoperability and usage of multiple programming languages within a large dataset of GitHub projects and Stack Overflow Q\&A. It addresses existing multi-lingual development practices and interactions between programming languages, focusing on in-process multi-programming language interoperability. The research examines a dataset of 414,486 GitHub repositories, 22,156,001 Stack Overflow questions from 2008-2021 and 173 interoperability tools. The paper's contributions include a comprehensive dataset, large-scale analysis, and insights into the prevalence, dominant languages, interoperability tools, and related issues in multi-language programming. The paper presents the research results, shows that C is a central pillar in programming language interoperability, and outlines \emph{simple interoperability} guidelines. These findings and guidelines contribute to our multi-programming language interoperability system research, also laying the groundwork for other systems and tools by suggesting key features for future interoperability tools.

==> figures/clique_and_star.tex <==
\begin{figure}[h]
\centering
    \subfigure[Direct Binding]{
        \begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto] 
            \node[state]    (L1)                  {$L1$}; 
            \node[state]    (L2)   [right=of L1]  {$L2$}; 
            \node[state]    (L3)   [below=of L1]  {$L3$}; 
            \node[state]    (L4)   [right=of L3]  {$L4$}; 
            \path[<->]
            (L1) edge  node {}    (L2)
            (L1) edge  node {}    (L3)
            (L1) edge  node {}    (L4)
            (L2) edge  node {}    (L3)
            (L2) edge  node {}    (L4)
            (L3) edge  node {}    (L4)
            ; %end path 
        \end{tikzpicture}
        \label{fig:clique}
    }
    \qquad
    \subfigure[Indirect Binding]{
        \begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto] 
            \node[state]    (CodeSwitch)  [below=of L1]     {\smaller{CodeSwitch}}; 
            \node[state]    (L1)                            {$L1$}; 
            \node[state]    (L2)   [right=of CodeSwitch]    {$L2$}; 
            \node[state]    (L3)   [below=of CodeSwitch]    {$L3$}; 
            \node[state]    (L4)   [left=of CodeSwitch]     {$L4$}; 
            \path[<->]
            (L1) edge  node {}    (CodeSwitch)
            (L2) edge  node {}    (CodeSwitch)
            (L3) edge  node {}    (CodeSwitch)
            (L4) edge  node {}    (CodeSwitch)
            ; %end path 
        \end{tikzpicture}
        \label{fig:star}
    }
    \caption{Language Bindings}
\end{figure}

